Optimal Methods for Convex Risk Averse Distributed Optimization

This paper studies the communication complexity of convex risk-averse optimization over a network. The problem generalizes the well-studied risk-neutral finite-sum distributed optimization problem and its importance stems from the need to handle risk in an uncertain environment. For algorithms in the literature, there exists a gap in communication complexities for solving risk-averse and risk-neutral problems. We propose two distributed algorithms, namely the distributed risk averse optimization (DRAO) method and the distributed risk averse optimization with sliding (DRAO-S) method, to close the gap. Specifically, the DRAO method achieves the optimal communication complexity by assuming a certain saddle point subproblem can be easily solved in the server node. The DRAO-S method removes the strong assumption by introducing a novel saddle point sliding subroutine which only requires the projection over the ambiguity set $P$. We observe that the number of $P$-projections performed by DRAO-S is optimal. Moreover, we develop matching lower complexity bounds to show the communication complexities of both DRAO and DRAO-S to be improvable. Numerical experiments are conducted to demonstrate the encouraging empirical performance of the DRAO-S method.

==> centralize.tex <==
\section{Upper Bounds for Communication Complexity}

In this section, we consider a communication network with a star topology,
which has a computationally powerful server node and many worker nodes.
%such that the \textit{centralized communication} can be performed in $O(\Delta)$ communication rounds: 
All worker nodes send their local parameters to the central server and  the server node broadcasting parameters to all edge nodes. This type of distributed optimization
is very popular in machine learning, such as federated learning, where the central server
is usually defined as a parameter server.
In this section, we will present
our basic algorithmic schemes for solving
distributed smooth and nonsmooth risk averse optimization problems under the aforementioned star-topology setting.
%can be implemented if every communication link in the network have a large enough bandwidth.

\subsection{The algorithm and its convergence properties}
In this subsection, we first present a generic distributed
risk averse optimization (DRAO) algorithm and then specialize it for solving
smooth and nonsmooth problems. We also state a few upper bounds on the communication complexity associated with these algorithms. 


%\subsection{Convergence analysis}
We start with a generic distributed risk averse optimization (DRAO) algorithm for solving the min-max-max saddle point problem in \eqref{eq:prob}.
%and show that it can achieve the optimal communication complexity for both non-smooth and smooth problems.
{\bf Missing motivation of the algorithm. How does it relate
to SD and accelerated prox-level?}

As shown in Algorithm \ref{alg:cPD}, in DRAO the server first sends an extrapolated point $\xtilt$ to the workers for them to perform dual proximal updates in Line 3. The only goal is to reduce the component gap function $Q_{\pii}$. Notice that here we intentionally leave the prox-function $\Vi$ in an abstract form because its selection and the resulting implementation of the proximal update will depend on the smoothness properties of $\myfi$. Next, the server collects the newly generated $\piit$ to solve a well-structured saddle point problem so as to reduce both $Q_x$ and $Q_p$. 

%More specifically, we obtain the following convergence guarantee for Algorithm \ref{alg:cPD}.


%\subsection{Centralized Primal Dual Algorithm} 
\begin{minipage}{1\textwidth}
\begin{algorithm}[H]
\caption{A generic distributed risk averse optimization (DRAO) algorithm}
\label{alg:cPD}
\begin{algorithmic}[1]
\Require $\xt[0]=\xt[-1] \in X$, $\piit[0] \in \Pii $ in every node, stepsizes $\{\thetat\}$, $\{\etat\}$, $\{\taut\}$, and  weights $\{\wt\}$.

\For{$t =  1,2,3 ... N$}
\parState{Server computes $\xtilt\leftarrow \xtt + \thetat (\xtt - \xt[t-2])$. Broadcast it to all workers.}
\parState{Every worker computes $\piit \leftarrow \argmax_{\pii \in \Pii} \inner{\xtilt}{\pii} - \fistar(\pii) - \taut V_i(\pii; \piitt)$ and $\fistar(\piit)$.}
\parState{All workers send their $(\piit, \fistar(\piit))$ to the server.}
\parState{Server updates $\xt \leftarrow \argmin_{x \in X} \max_{p \in P} \sumi p_i (\inner{x}{\piit} - \fistar(\piit)) + \tfrac{\eta}{2} \normsq{x - \xtt}.$ {\bf I suggest to use general Bregman distance rather than Euclidean distance for the primal updates.}}
\EndFor
\State \Return $\xbart[N]:= \tsum_{t=1}^N \wt \xt / (\sumt \wt). $
\end{algorithmic}
\end{algorithm}
\end{minipage}


Observe that in the generic DRAO algorithm, we assume that
the subproblems in step 3 and 5 can be solved
exactly by the workers and server, respectively.
In fact, step 3 reduces to local gradient evaluations in the smooth case, while requiring an
iterative procedure for the general nonsmooth case.
Step 5 requires us to solve a structured bilinear saddle 
point problem. We will discuss in more details
how to solve these problems approximately in next Section, while focusing on the communication complexity in this section.

%Under the centralized setting, we choose to carry out the majority of computation in the central node while utilizing edge nodes only for tasks similar to local gradient evaluations.

\vgap

We now consider a class of smooth risk averse optimization for which all $\myfi$'s are smooth s.t.
\[
\| \nabla \myfi(x_1) - \nabla \myfi(x_2)\|_* \le L_i \|x_1 - x_2\|, \forall x_1, x_2 \in X.
\]
In this case,
a natural choice of the prox-function $\Vi$ in DRAO would be the Bregman distance function generated by $\fistar:$
\begin{equation} \label{eq:dual_bregman}
\Dfistar(\pii; \bpii) := \fistar(\pii) - \fistar(\bpii) - \inner{\fistarp(\bpii)}{\pii - \bpii}.
\end{equation}
It has been shown in~\cite{LanZhou18RPDG,LanBook,zhang2020optimal} that
the dual proximal update in Line 3 of Algorithm \ref{alg:cPD} is equivalent to a gradient evaluation. Specifically, Line 3 reduces to
\begin{align}
    \xundert &\leftarrow (\xundert[t-1] + \taut \xtilt)/(1 + \taut),\label{eq:smooth_alg1}\\
    \piit &\leftarrow \grad \myfi(\xundert),\label{eq:smooth_alg2}\\
    \fistar(\piit)&\leftarrow  \inner{\xundert }{\piit}- \myfi(\xundert).\label{eq:smooth_alg3}
\end{align}
Plugging $\fistar(\piit)$ defined in \eqref{eq:smooth_alg3} into Line 5 of Algorithm~\ref{alg:cPD}, we can completely remove any information about
the conjugate function $f^*$. Therefore, DRAO is considered to be a purely primal algorithm for smooth risk averse optimization.

To discuss the convergence properties of DRAO for smooth problems, we need to properly define some Lipschitz constants. For a given $p \in P$, let us denote $f_p(x) := \sumi p_i f_i(x)$.
Clearly $f_p$ is a smooth convex function with Lipschitz continuous gradients
s.t.
\[
\|\nabla f_p(x_1) - \nabla f_p(x_2)\|_* \le L_p \|x_1 - x_2\|, \forall x_1, x_2 \in X. 
\]
Moreover, we have $L_p \le \sumi p_i L_i$. We then define the following constant $\Lf$  to characterize the overall smoothness of the risk averse problem \eqref{eq:prob}:
\begin{equation}\label{eq:smo_cst}
\Lf = \max_{p \in P} L_p.
\end{equation}
 Observe that in the risk neutral case where $P=\{(1/m,\ldots,1/m)\},$ $\Lf$ is the global smoothness constant of $f$, which is bounded by $\tfrac{1}{m} \sumi L_i$.
% \cite{scaman2017optimal}, 
 Moreover, in the robust case when $P= \Delta_m^+$, $\Lf \le \max_i L_i$.
 
 Theorem~\ref{thm:central-sm} shows the convergence rate of the DRAO method applied to the aforementioned smooth problems.
 The proof of this result is given in Section~\ref{sec:ConvergenceAnalysis}.
 \begin{theorem}\label{thm:central-sm}
% Consider the DRAO method applied to smooth problem.
%Let $\{\myfi\}$ be smooth with an aggregate smoothness constant $\Lf$ defined in \eqref{eq:smo_cst}. 
Let $\{\xt\}$ be generated by the DRAO method applied to smooth problems with
$$\wt=t/2,\ \thetat=(t-1)/(t), \taut = (t-1)/2, \etat = 2\Lf/t,$$
where $\Lf$ is defined in \eqref{eq:smo_cst}, then we have the following inequality for any $\hz:=(\hx; \hp, \hpiibr)$ with $\hpii = \grad \myfi(x)$ for some $x\in X$,
\begin{equation}\label{eq:smooth_Q_conv}
\sumt \wt Q(\zt; \hz) + 2\Lf \normsq{\xt[N] - \hx} \leq 2\Lf \normsq{\xt[N] - \hx}.\end{equation}
In particular the ergodic solution $\xbart[N]$ satisfies 
\begin{equation}\label{eq:smooth_f_conv}
f(\xbart[N]) - f(\xstar) \leq 2\Lf \normsq{\xt[N] - \xstar}/N^2.\end{equation}
\end{theorem}

Notice that if $\hz$ in \eqref{eq:smooth_Q_conv} is chosen to be the saddle point defined in Lemma \ref{lm:sad_ex}, the preceding theorem implies that $\xt$ is always inside an $\norm{\xt[0] - \xstar}$ ball around $\xstar$, i.e., 
$$\norm{\xt - \xstar} \leq \norm{\xt[0] - \xstar} \ \forall t.$$
Moreover, since each iteration of Algorithm \ref{alg:cPD} require $\bigO(\Delta)$ communication rounds, its communication complexity is $\bigO(\Delta\Lf\normsq{\xt[0] - \xstar}/\sqrt{\ep})$, matching the lower bound of a centralized risk-neutral smooth example shown in \cite{scaman2017optimal}.

In view of Theorem~\ref{thm:central-sm},
the total number of communication rounds required to find an $\epsilon$-solution
of problem~\eqref{eq:orig_prob} can be bounded by ${\cal O}(1/\sqrt{\epsilon})$.
We will show later in Section~3 that this bound is not improvable in general.



%\begin{minipage}{1\textwidth}
%\begin{algorithm}[H]
%\caption{Concrete Implementation of Line 3 in the cPD Algorithm \ref{alg:cPD} for %Smooth $\myfi$}
%\label{alg:smooth_cPD}
%\begin{algorithmic}[1]
%\Require $\dots$ Set $\xundert[0] %\leftarrow \xt[0]. $
%\For{$t =  1,2,3 ... N$}
%\State $\vdots$
%\parState{Every node computes %$\xundert\leftarrow (\xundert[t-1] + \taut \xtilt)/(1 + \taut).$\\
%Set $\piit \leftarrow \grad \myfi(\xundert)$ and $\fistar(\piit)\leftarrow  \inner{\xundert }{\piit}- \myfi(\xundert)$.}
%\State $\vdots$
%\EndFor
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}



\vgap

When the local cost functions $\myfi$ are non-smooth, the previously chosen prox-function $\Dfistar$ (c.f. \eqref{eq:dual_bregman}) is no longer suitable, because $\myfi^*$ may not be strongly convex. Instead we choose
$\Vi(\pii; \bpii):= \tfrac{1}{2} \normsq{\pii - \bpii},$
and assume that the workers can carry out the following proximal update for any scalar $\tau>0$ and $u\in \R^n$ between communications,
$$\uy \in \argmin_{y} \myfi(y) + \tfrac{1}{2\tau} \normsq{y - u}.$$
In particular, we replace step 3 of Algorithm~\ref{alg:cPD} 
by 
\begin{align}
    \uyit &\leftarrow \argmin_{y} f(y) + \tfrac{1}{2\taut} \normsq{\xtilt + \taut \piitt - y}, \label{eq:nonsmooth_alg1}\\
 \piit &\leftarrow \piitt + \tfrac{1}{\tau} (\xtilt -\uyit),\label{eq:nonsmooth_alg2}\\ 
 \fistar(\piit)&\leftarrow  \inner{\uyit }{\piit}- \myfi(\uyit).\label{eq:nonsmooth_alg3}
\end{align}
The following lemma verifies that \eqref{eq:nonsmooth_alg1}-\eqref{eq:nonsmooth_alg3} 
correspond to a correct implementation of Step 3 of Algorithm~\ref{alg:cPD}.

\begin{lemma}
Let $(\uyit,\piit)$ be defined in \eqref{eq:nonsmooth_alg1}-\eqref{eq:nonsmooth_alg2} and $\fitilstar(\piit):= \inner{\uyit }{\piit}- \myfi(\uyit)$. Then they satisfy
\begin{equation}\label{eq:non-smooth-orimal-reform}
\piit = \argmax_{\pii \in \Pii} \inner{\xtilt}{\pii} - \fistar(\pii) - \tfrac{\taut}{2} \normsq{\pii -\piitt} \text{ and } \fitilstar(\piit) = \fistar(\piit.)\end{equation}
\end{lemma}

\begin{proof}
Let us fix an $i \in [m]$ and let $\bu:=\xtilt + \taut \piitt$. Consider the Moreau envelop of $f$ given by %\cite{Beck2017First},
$g(u):= \inf_{y} f(y) + \tfrac{1}{2\tau} \normsq{u - y}.$
Since $f$ is convex, $g$ is convex and smooth over $\R^n$, thus $\partial g(\bu)$ is non-empty and unique.
Next, let $\bg(u):= f(\uyit) + \tfrac{1}{2\tau} \|u - \uyit\|^2.$
Since $\uyit := \inf_{y} f(y) + \tfrac{1}{2\tau} \normsq{\bu - y}$ in Algorithm \ref{alg:nonsmooth_cPD}, we have 
$g(\bu) = \bg(\bu)$ and $g(u) \leq \bg(u)$, thus the subgradient of $g$ at $\bu$ must be a subgradient of $\bg$ at $\bu$, i.e.,
$$\partial g(\bu) \subset \partial \bg(\bu) = \{\piit := \tfrac{1}{\tau}(\bu - \uyit)\}.$$
Therefore $\piit = \grad g(\bu).$
%As shown below, 
%\eqref{eq:non-smooth-orimal-reform} 
It then follows from the Fenchel conjugate duality and the identity, ({\bf the notation $\Box$ has not been defined})
$$(g)^*(\pii) =(f \Box \tfrac{1}{2\taut}\normsq{\cdot})^*(\pii)=\fistar(\pii) + \tfrac{\taut}{2}\normsq{\pii}\ \forall \pii.$$
that
\begin{align*}
\piit \in \partial (f \Box \tfrac{1}{2\taut}\normsq{\cdot})(\bu) 
%&\Leftrightarrow \bu \in \partial  (f \Box \tfrac{1}{2\taut}\normsq{\cdot})^*(\piit)\\
&\Leftrightarrow \piit \in \argmax_{\pii} \inner{\bu}{\pii} - (f \Box \tfrac{1}{2\taut}\normsq{\cdot})^*(\pii)\\
&\Leftrightarrow \piit \in  \argmax_{\pii \in \Pii} \inner{\xtilt}{\pii} - \fistar(\pii) - \tfrac{\taut}{2} \normsq{\pii -\piitt},
\end{align*}
where the last equivalence follows from the definition of $\bu.$
Moreover, the first-order optimality condition for $\uyit$ implies that $\piit = \tfrac{1}{\tau}(\bu - \uyit) \in \partial \myfi(\uyit)$. Thus it follows from the Fenchel conjugate duality that
$\fistar(\piit) = \inner{\piit}{\uyit} - \myfi(\uyit).$
\end{proof}

Observe that in this section we assume subproblems \eqref{eq:nonsmooth_alg1} can be solved exactly. This happens when $\myfi$ is relatively simple (e.g., $l_1$ norm). Otherwise, we need to apply an iterative procedure to solve these subproblems (see Section 4). For both these cases, the server does not have direct access to $\myfi$. Also note that similar to the smooth case, with the definition of $\fitilstar(\piit)$ in \eqref{eq:nonsmooth_alg3}
the workers do not really need to have access to the conjugate functions $\fitilstar(\cdot)$. 

Theorem~\ref{thm:cen-non-smooth} below states the convergence properties of Algorithm \ref{alg:cPD} applied to nonsmooth problems, and its proof is provided in Section~\ref{sec:ConvergenceAnalysis}. For these We assume that each local cost function is Lipschitz continuous s.t. $\max_{x \in X} \|f'_i(x)\| \le M_i$. 
We also define Lipschitz constant $\Mfbar$ as 
%the maximum $p-$weighted $l_2$ norm of the sub-gradients of $\{\myfi\}$
\begin{equation}\label{eq:Mf_def}
\Mfbar  = \max_{x} \max_{p \in P}  \left(\sumi p_i \normsq{\myfi'(x)}\right)^{1/2}.
\end{equation}
Clearly we have 
\[
\Mfbar \le \max_{p \in P} \left(\sumi p_i M_i^2\right)^{1/2} \le \max_{i=1,\ldots,m} M_i.
\]
% It is worth noting that $\Mfbar$ is larger than  the Lipschitz constant $\Mf :=\max_{p \in P}\{\text{Lipschitz continuity constant of } \sumi p_i \myfi\},$ which shows up in the convergence bounds for $O(1/\ep^2)$ algorithms, e.g., the gradient descent method. Such a discrepancy arises because we are essentially ``smoothening'' \cite{Nestrov2004Smooth}  $\{\myfi\}$ and the aggregate gradient of the smoothed functions could be quite different from the aggregate gradient of the non-smooth $\{\myfi\}$.

\begin{theorem}\label{thm:cen-non-smooth}
%Let $\{\myfi\}$ be non-smooth and their aggregate Lipschitz continuity constant $\Mfbar$ defined in \eqref{eq:Mf_def}. 
Let $\{\xbarN\}$ be generated by the DRAO method applied to nonsmooth problems
with 
$$\wt=1,\ \thetat=1, \etat = \Mfbar / (2\norm{x_0 - \xstar}), \taut = 2\Mfbar / \norm{x_0 - \xstar},$$
where $\Mfbar$ is defined in \eqref{eq:Mf_def},
then 
\begin{equation}\label{eq:nonsmooth_f_conv}
f(\xbart[N]) - f(\xstar) \leq 2\Mfbar \normsq{\xt[N] - \xstar}/N.\end{equation}
\end{theorem}

The preceding theorem gives us an $\bigO(\Delta\norm{\xt[0] - \xstar}\Mfbar/\ep)$ communication complexity for solving distributed nonsmooth risk averse  problems.

\subsection{Convergence analysis} \label{sec:ConvergenceAnalysis}

Our main goal in this subsection is to establish the convergence rates associated with the DRAO method stated in Theorems~\ref{thm:central-sm} and \ref{thm:cen-non-smooth}.

\vgap

We will first show some general convergence properties about the generic DRAO method in Algorithm~\ref{alg:cPD}. Notice that
this result holds regardless of the strong convexity of $\fistar$ (i.e., $\mu = 0$ is allowed in \eqref{eq:strong_convex_dual}), and thus can be applied to both smooth and nonsmooth problems.

\begin{proposition}\label{pr:central_Q_conv}
Let $\{\zt \equiv (\xt; \pt,\pi^t) \}$ be generated by Algorithm~\ref{alg:cPD} with some $\pt\in \argmax_{p \in P} \sumi p_i (\inner{\xt}{\piit} - \fistar(\piit))$. Assume that 
$\fistar$ satisfy 
\begin{equation} \label{eq:strong_convex_dual}
\fistar(\pii) - \fistar(\bpii)- \inner{\fistarp(\bpii)}{\pii - \bpii} \geq \mu \Vi(\pii; \bpii),\ \forall \pii, \bpii \in \Pii
\end{equation}
for some $\mu \ge 0$.
If the stepsizes satisfy 
%$$\wtt=\wt\thetat,\ \wt \etat \leq \wtt \etatt, \wt\taut \leq \wtt (\tautt  + \mu), $$ 
\begin{align*}
\wtt=\wt\thetat,\ \wt \etat \leq& \wtt \etatt, \wt\taut \leq \wtt (\tautt  + \mu),\\
\wt \taut \sumi \hpi \Vi(\piit; \piitt) + \tfrac{\wtt\etatt}{2}\normsq{\xtt - \xt[t-2]} &\geq \wtt \sumi \hpi \inner{\piitt - \piit}{\xtt - \xt[t-2]}, \forall t\in [N],\\
\wt[N] (\taut[N]+\mu) \sumi \hpi \Vi(\hpii; \piit[N-1]) + \tfrac{\wt[N]\etat[N]}{2}\normsq{\xt[N] - \xt[N-1]} &\geq \wt[N] \sumi \hpi \inner{\piit[N] - \hpii}{\xt[N-1] - \xt[N]},
\end{align*}
then we have for all $\hz:=(\hx; \hp, \hat \pi) \in X \times P \times \Pi$,
\begin{equation}\label{eq:central_Q}
\sumt \wt Q(\zt; \hz) + \tfrac{\wt[N] \etat[N]}{2} \normsq{\xt[N] - \hx} \leq \tfrac{\wt[1] \etat[1]}{2} \normsq{\xt[0] - \hx} + \wt[1]\taut[1]\sumi \hpi \Vi(\hpii; \piit[0]).
\end{equation}
\end{proposition}

\begin{proof}
Let $Q_\pi$, $Q_p$ and $Q_x$ be defined in \eqref{eq:Q-decomp}.
We begin by analyzing the convergence of $\Q[\pii](\hz; \zt).$ It follows from the definition of $\xtilt$ that
\begin{align*}
\inner{\hpii -\piit }{\xtilt-\xt}=& -\inner{\hpii - \piit}{\xt -\xtt} + \thetat \inner{\hpii -\piitt}{\xtt -\xt[t-2]}\\
&+\thetat \inner{\piitt -\piit}{\xtt -\xt[t-2]}.
\end{align*}
By the optimality condition for the dual update in Line 3
of ALgorithm~\ref{alg:cPD} (see Lemma 3.1 of \cite{LanBook}), we have
\begin{align*}
\inner{\hpii - \piit}{\xt}& + \fistar(\piit) - \fistar(\hpii) + \inner{\hpii -\piit }{\xtilt-\xt} \\
&\leq \taut \Vi(\hpii; \piitt) - (\taut + \mu) \Vi(\hpii; \piit) - \taut \Vi(\piit; \piitt).
\end{align*}
Combining the above two relations,
taking the $\wt$ weighted sum of the resulting inequalities and using the conditions that $\wtt=\wt\thetat$ and $\wt\taut \leq \wtt (\tautt  + \mu)$, we obtain 
\begin{align*}
\sumt \wt &(\inner{\hpii - \piit}{\xt} + \fistar(\piit) - \fistar(\hpii)) \\
\leq& - (\wt[N](\taut[N] + \mu) \Vi(\hpii; \piit) -\wt[N]\inner{\hpii - \piit[N]}{\xt[N] -\xt[N-1]})\\
& -\tsum_{t=2}^{N} [\wt \taut \Vi(\piit; \piitt) + \wtt \inner{\piitt -\piit}{\xtt -\xt[t-2]} ]\\
&+ \wt[1]\taut[1] \Vi(\hpii; \piit[0]) 
\end{align*}
Then summing up all the $i$s with weight $\hpi$, we get 
\begin{align}\label{eq:central_Qpii_bound}
\begin{split}
\sumt \wt& Q_\pi(\zt;\hz) \\
\leq& - (\wt[N](\taut[N] + \mu) \sumi \hpi \Vi(\hpii; \piit) -\wt[N]\inner{\sumi \hpi(\hpii - \piit[N])}{\xt[N] -\xt[N-1]})\\
& -\tsum_{t=2}^N [\wt \taut\sumi \hpi \Vi(\piit; \piitt) + \wtt \inner{\sumi \hpi(\piitt -\piit)}{\xtt -\xt[t-2]} ]\\
&+ \wt[1]\taut[1] \Vi(\hpii; \piit[0]) .
\end{split}
\end{align}

Next, we consider the $\xt$ and $\pt$ generated by Line 5 in Algorithm \ref{alg:cPD}. Denote the proximal sub-problem by 
$$F(x; \piitbr):= \max_{p \in P}\sumi p_i (\inner{x}{\piit} - \fistar(\piit)) + \tfrac{\eta}{2} \normsq{x - \xtt}.$$
Since any $p\in P$ is always (componentwise) non-negative, $F(x;\piitbr)$ is a convex function. Thus the first order optimality condition for $\xt$ implies the existence of some $\pt$ for which 
\begin{equation*}
\begin{split}
\pt \in& \argmax_{p \in P} \sumi p_i (\inner{\xt}{\piit} - \fistar(\piit)) + \tfrac{\eta}{2} \normsq{\xt - \xtt} \\
&\Rightarrow \sumi (\hpi - p^t) (\inner{\xt}{\piit} - \fistar(\piit))\leq 0 \Rightarrow Q_p(\zt;\hz) \leq 0.
\end{split}\end{equation*}
Moreover,
\begin{equation*}
\sumi \pt_i \piit + \eta (\xt - \xtt) \in -\partial \delta_X(\xt) \Rightarrow  \inner{\sumi \pt_i \piit + \etat (\xt - \xtt)}{\xt- \hx} \leq 0,\ i.e.,
\end{equation*}
\begin{equation*}
\Q[x](\zt;\hz) + \tfrac{\etat}{2} \normsq{\xt - \hx} \leq \tfrac{\etat}{2} \normsq{\xtt - \hx} - \tfrac{\etat}{2} \normsq{\xt - \xtt}
\end{equation*}
({\bf This part needs to be revised for general Bregman distance})
Summing up  the above $\Q[x]$ and $\Q[p]$ inequalities ({\bf give these inequalities a number so that you can refer t them }) with weight $\wt$ and noticing $\wt\etat \leq \wtt \etatt$, we obtain
\begin{equation}\label{eq:central_Qx_Qp}
\sumt \wt (\Q[x](\zt; \hz)+\Q[x](\zt; \hz)) + \tfrac{\wt[N]\etat[N]}{2} \normsq{\xt[N] - \hx} \leq \tfrac{\wt[1]\etat[1]}{2} \normsq{\xt[0] - \hx} - \sumt \tfrac{\wt\etat}{2} \normsq{\xt - \xtt}.
\end{equation}
Then we can conclude \eqref{eq:central_Q} by adding \eqref{eq:central_Qx_Qp} to \eqref{eq:central_Qpii_bound}.
\end{proof}

%\subsection{Smooth Local Cost Functions}\label{subsec:cen_sm}

We now specialize the results obtained in Proposition~\ref{pr:central_Q_conv} for the smooth problems.
 Observe that the gradient evaluation point $\xundert$ is common for all workers. This allows us to easily characterize the strong convexity modulus of the aggregate dual prox-functions $\sumi \hpi \Dfistar(\cdot;\cdot)$ in the next lemma. ({\bf Typo in $\Dfistar$. The suberscript should be $i$.})
\begin{lemma}\label{lm:agg_sm}
Let $\hp\in P$ be given. If $\pii = \grad \myfi(x) $ and $\bpii = \grad \myfi(\xbar)$ for some $x$ and $\xbar$, then 
\begin{equation}
\sumi \hpi \Dfistar(\pii;\bpii) \geq \tfrac{1}{2\Lf}\normsq{\sumi \hpi(\pii - \bpii)}.
\end{equation}
\end{lemma}

\begin{proof}
Let $\myfi[\hp](x):=(\sumi \hpi \myfi(x)).$ Then by the definition of $\Lf$ in \eqref{eq:smo_cst}, $\myfi[\hp]$ is $\Lf$-smooth and its conjugate $(\myfi[\hp])^*$ is $1/\Lf$ strongly convex. 
Next, we relate  $D_{(\myfi[\hp])^*}$ to $\sumi \hpi \Dfistar(\cdot;\cdot)$ to calculate its strong convexity modulus. Since 
$$\sumi \hpi \pii \in \grad \myfi[\hp](x), \sumi \hpi \bpii \in \grad \myfi[\hp](\xbar),$$
we have by the Fenchel duality that
$$\sumi \hpi \inner{\pii -\bpii}{\grad \fistar(\bpii)} =  \inner{\sumi \hpi (\pii -\bpii)}{\xbar} = \inner{\sumi \hpi (\pii -\bpii)}{\grad (\myfi[\hp])^*(\sumi \hpi \bpii) }\},
$$
$$\sumi \hpi \fistar(\pii) = \sumi \hpi (\inner{\pii}{x} - \myfi(x)) = \inner{\sumi \hpi\pii}{x} - (\sumi \hpi \myfi)(x) = (\myfi[\hp])^*(\sumi \hpi\pii),$$
and hence
$$\sumi \hpi \fistar(\bpii) =  (\myfi[\hp])^*(\sumi \hpi\bpii).$$
Thus 
$$\sumi \hpi \Dfistar(\pii;\bpii) = D_{(\myfi[\hp])^*}(\sumi \hpi\pii;\sumi \hpi\bpii) \geq \tfrac{1}{2\Lf}\normsq{\sumi \hpi(\pii - \bpii)},$$
where the last inequality follows from the strong convexity of $(\myfi[\hp])^*$.
\end{proof}

\vgap

We are now ready to prove Theorems~\ref{thm:central-sm} and \ref{thm:cen-non-smooth}.

\vgap

\noindent{\bf Proof of Theorem~\ref{thm:central-sm}:}
%\begin{proof}
First, notice that $\fistar$ is $1$-strongly convex with respect to $\Dfistar$. Then is easy to verify that our stepsize choices, together with the $1/\Lf$ strong convexity of $\sumi \hp \Dfistar$ (for $\piibr$ and $\hpii$) shown in Lemma \ref{lm:agg_sm}, satisfy all the requirements in Proposition \ref{pr:central_Q_conv}. Thus \eqref{eq:smooth_Q_conv} follows as a consequence of it. 

Next, let $\hpiiN = \grad \myfi(\xbart[N])$ and $\hpiN[] \in \argmax_{p \in P} \sumi p_i \myfi(\xbart[N])$ such that $f(\xbarN)= \La(\xbarN; \hpiN, \hpiiN)$ (shown in Lemma \ref{lm:duality}). We choose $\hz:= (\xstar;\hpN, \hpiiNbr)$ in \eqref{eq:smooth_Q_conv} such that 
$$\sumt \wt \La(\xt; \hpN, \hpiiNbr) - \sumt \wt \La(\xstar; \pt, \piitbr) \leq 2\Lf \normsq{\xt[N] - \xstar}. $$
The linearity of $\La(\cdot; \hpN, \hpiiNbr)$ with respect to $x$ and the weak duality in Lemma \ref{lm:duality} implies that 
$$\sumt \wt \La(\xt; \hpN, \hpiiNbr) = \tfrac{N(N+1)}{4} \La(\xbarN; \hpN, \hpiiNbr) = \tfrac{N(N+1)}{4} f(\xbarN), $$
and that
$$\sumt \wt \La(\xstar; \pt, \piitbr) \leq \tfrac{N(N+1)}{4} f(\xstar).$$
Therefore, \eqref{eq:smooth_f_conv} follows from combining the preceding three relations.

\endproof

\vgap

\noindent{\bf Proof of Theorem~\ref{thm:cen-non-smooth}}
It is easy verify that the requirements in Proposition \ref{pr:central_Q_conv} is satisfied, thus for any feasible $\hz$, we have
$$\sumt \wt Q(\zt; \hz) + \tfrac{\wt[N] \etat[N]}{2} \normsq{\xt[N] - \hx} \leq \tfrac{\wt[1] \etat[1]}{2} \normsq{\xt[N] - \hx} + \wt[1]\taut[1]\sumi \hpi \normsq{\hpii- \piit[0]}.$$
Next, let $\hpiiN = \grad \myfi(\xbart[N])$ and $\hpiN[] \in \argmax_{p \in P} \sumi p_i \myfi(\xbart[N])$ such that $f(\xbarN)= \La(\xbarN; \hpiN, \hpiiN)$ and set $\hz = (\xstar; \hpN, \hpiiNbr)$, we get 
$$\sumt \wt Q(\zt; \hz)  \leq \tfrac{\etat[1]}{2} \normsq{\xt[N] - \xstar} + 2\taut[1]\Mfbar^2 = 2 \norm{\xt[N] - \xstar}\Mfbar.$$
Then we can conclude \eqref{eq:nonsmooth_f_conv} by applying the same function value gap argument in Theorem \ref{thm:central-sm}.

\endproof


\section{Lower Bounds on Communication Complexity}

The lower bound depends a notion of network black-box optimization procedure inspired by \cite{scaman2017optimal}. More specifically, an algorithm is said to be a network black-box optimization procedure if it satisfies the following requirements:
\begin{enumerate}
\item \textbf{Local memory:} each node $i$ store past iterates in a (finite) local memory $\Mit\subset \R^n$ at time $t$. Between each communication round, $\Mit$ can be updated by either communicating with neighboring nodes or by performing further local computation:
$$\Mit \subset \Mitcp \cup \Mitcm.$$
\item \textbf{Local computation:} each node can carry out multiple turns of local computation between communication rounds:
$$\Mitcp = \Mit^L, \text{ where } \Mit^0 = \Mit[t-1], \ \Mit^l \subset \Span(\{x, \partial f_i(x), \prox_{\myfi}(x;\tau): x\in \Mit^{l-1}, \tau > 0\}),$$
where $\prox_{\myfi}(x;\tau):= \argmin_{y} \myfi(y) + \tau/2 \normsq{y - x}.$
\item \textbf{Local communication:} at communication round $t$, each node can share internal iterates with all its neighbors:
$$\Mitcm \subset \Span(\cup_{j \in \mathcal{N}(i)} \Mit[t-1][j]).$$
\item \textbf{Output value:} at communication round $t$, the network outputs some iterate from some node's local memory:
$$\xt \in \cup_{i\in[m]} \Mit.$$

\end{enumerate}

We make two remarks regarding the requirements. First, in contrast to \cite{scaman19} where one turn of gradient evaluation is permitted, we allow many turns of both proximal updates and gradient computations. We choose the stronger local computation model to highlight the communication bottleneck. Second, communicating function value  
is superfluous because an arbitrary selection of elements in the generated linear space is allowed in both the local communication and computation step ({\bf no sure what you mean here.}). In particular, Line 5 of Algorithm \ref{alg:cPD} amounts to just one turn of local computation after all $\piit$ is passed to the central node since 
 $$\xt = \xtt - \sumi \hpi \piit/\eta \text{ for some $\hpi\in\R$}.$$
 Therefore Algorithm \ref{alg:cPD} is but one black-box optimization procedure. 

 \begin{figure}[!htb]
\centering
    \begin{minipage}{0.5\textwidth}
        % \centering
          \begin{tikzpicture}[auto,node distance=8mm,>=latex,font=\small]
            % \draw[help lines] (0,-5) grid (15,5);
            \tikzstyle{round}=[thick,draw=black,circle]
            \tikzstyle{rect}=[thick,draw=black,rectangle]

            \draw[->] (0,0) -- (6,0) node[anchor=north west] {$x$};
            \draw[->] (3,0) -- (3,2.5) node[anchor=south east] {$\sigma(x;\alpha)$};
            \draw[ultra thick, orange] (0,1.5) -- (1.5, 0);
            \draw[thick, orange, dashed] (1.5 ,0) -- (2.5, -1);
            \draw[ultra thick, orange] (1.5, 0) -- (4.5, 0);
            \draw[ultra thick, orange] (4.5, 0) -- (6, 1.5);
            \draw[thick, orange, dashed] (3.5, -1) -- (4.5, 0);

             \draw (1.5 cm , 1pt) --  (1.5 cm , -1pt) node[anchor=north] {$-\alpha$};
             \draw (4.5 cm , 1pt) --  (4.5 cm , -1pt) node[anchor=north] {$-\alpha$};

             \node[below] at (3,0) {$\sigma_2(x)=0$};
             \node[right] at (0,1.5) {$\sigma_1(x)=-x+\alpha$};
             \node[left] at (6,1.5) {$\sigma_3(x)=x-\alpha$};

           % \draw[thick] (3.3, 0.6)--(4.3, 0.6);
           % \node[below] at (3.8, 0.6) {\scriptsize $l(z):=z_1$};
        \end{tikzpicture}
        % \caption{\scriptsize Illustration $\sigma(x;\alpha)$ function.}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
    $
        \sigma(x; \alpha) := \max \begin{cases} \sigma_1(x)=-x+\alpha \\
        \sigma_2(x)=0 \\
        \sigma_3(x)=x-\alpha.
        \end{cases}
    $
    \end{minipage}

\caption{Illustration of $\sigma(x;\alpha)$ function.}\label{fig:sigma}
\end{figure}
\begin{figure}[!htb]
\begin{minipage}{0.5\textwidth}
          \begin{tikzpicture}[auto,node distance=8mm,>=latex,font=\small]
            % \draw[help lines] (0,-5) grid (15,5);
            \tikzstyle{round}=[thick,draw=black,circle]
            \tikzstyle{rect}=[thick,draw=black,rectangle]

            \node[round] (f1) {$f_{0\ \ \ }$};
            \node[round,fill=gray, right=1 of f1] (f2) {$f_{1\ \ \ }$};
            \node[right=1 of f2] (d) {$...$};
            \node[round, right=1 of d,fill=gray] (fmm) {$f_{m-1}$};
            \node[round, right=1 of fmm] (fm) {$f_{m\ \ \ }$};
            \draw[-] (f1)--(f2);
            \draw[-] (f2)--(d);
            \draw[-] (d)--(fmm);
            \draw[-] (fm)--(fmm);
        \end{tikzpicture}
\end{minipage}
\hfill
    \begin{minipage}{0.4\textwidth}
    \small
    \begin{align*}
    f&(x):= \max_{p \in \Delta_{+}} \sumi p_i \myfi(x),\text{    where }\\  
            &f_i(x):=0\ \forall 1<i<m, \\
            &f_0(x):=  \beta(\sigma(x_{1})+ 2 \tsum_{i=1}^{n/2} \sigma(x_{2i} - x_{2i-1}; \alpha) - x_n), \\
            &f_m(x):= \beta(\sigma(x_1)+2  \tsum_{i=1}^{n/2} \sigma(x_{2i+1} - x_{2i}; \alpha) - x_n). 
        \end{align*}
    \end{minipage}
    \caption{Hard Network Instance for Non-Smooth Problem}
    \label{fig:ns_hard}
\end{figure}
 Next we suggest a hard instance parametrized by $m,n,\beta, \alpha$. More specifically, as illustrated in Figure \ref{fig:ns_hard}, the instance consists of a linear network of size $m$, a decision variable of an even size $n$, $x \in X := \R^n$, trivial functions at the middle nodes and alternating functions at the head and the tail node. Notice that this is also similar to 
the hard example in \cite{scaman19}. However instead of $\normsq{x}$ and $|x_i-x_{i-1}|$ in \cite{scaman19}, we use only piecewise linear function $\sigma(\cdot;\alpha)$ in Figure \ref{fig:sigma} for our construction. Such a piecewise linear function simplifies the analysis and comes handy analyzing decentralized procedures later. We provide below a lower bound for the optimality gap in $n/2$ communication rounds for any blackbox network optimization procedure. 


\begin{lemma}\label{lm:lower_ns}
Let $f$ be an hard instance shown in Figure \ref{fig:ns_hard}, specified according to some $(m, n, \alpha, \beta)$ with $n\geq 4$ being even, then 
$$\normsq{\xstar - \xt[0]} = \normsq{\xstar} \leq \alpha n^3/2,\text{ and } \MPi[] \leq 2 \beta \sqrt{n}.$$
Moreover, when applied to $f$ initialized with $\Mit[0]=\{0\}$, the output generated by any network black-box optimization procedure in $t < (n/2-1)m$ communication rounds must satisfy:
$$f(\xt) - f(\xstar) \geq n \alpha \beta /2.$$
\end{lemma}
\begin{proof}
The proof is based on showing that the iterates being confined to some subspace after only a limited number of communication rounds. Define $\Kl:=\{x \in R^n: x_j =0, \forall j \leq n-l\}$. Then we obtain the following constraints on $\Mitcp$ if $\Mit[t-1] \subset \Kl:$
$$\Mitcp \subset \begin{cases}\Kl &\text{if } i=0, l \text{ is odd}\\
\Kl &\text{if } i=m, l \text{ is even}\\
\Kl &\text{if  } 1<i < m.
\end{cases}$$
Thus for an odd $l$, the only way for $\Mit[t][1]$ to include any element of $\Kl[l+1]/\Kl$ is to receive one from communicating with a neighboring node. After that, a gradient evaluation at node $1$ leads to some element in  $\Kl[l+2]/\Kl[l+1].$ Such an observation leads us to the following claim which can be shown via induction:
$$\Mt:=\cup_{i \in [m]} \Mit \subset \Kl[l+1], \forall t \leq ml -1.$$

We sketch the induction argument. When $l=1$, the claim clearly holds because $\Mit[t][0]\subset\Kl[2]$, and $\Mit[t][m]\subset \Kl[1]$ because any vector with an non-zero $n-1$ index in $\Mit[0][0]$ takes $m$ communication rounds to reach node $m$. Next, under the induction hypothesis, a similar argument shows that it takes $m$ communication rounds to increment the possible subspace of $\Mt$ by one dimension. 

Therefore, we must have $\Mt\subset \Kl[n/2]$ for $t <(n/2-1)m$ communication rounds. It remains to calculate the minimum possible optimal gap. We use a lower approximation to $f$ to aide the calculation:
$$\tilde{f}(x) := \tfrac{1}{2}\myfi[0](x) + \tfrac{1}{2}\myfi[m](x)= \beta (\sigma(x_1; \alpha) + \sum_{j=1}^{n-1} \sigma(x_{i+1} - x_{i};\alpha) - x_n),$$
  With the following change of variable,
$$d\in \R^n \text{ with } d_1 = x_1 \text{ and } d_j =x_{j} - x_{j-1} \forall 1<j \leq n,$$
it is easy to see that $\bar{f}(d) = \tilde{f}(x)= \beta(\sum_{j=1}^{n} \sigma(d_j;\alpha) - d_j)$. Thus the optimal is achieved at 
$$d=(\alpha, \alpha, \ldots,\alpha) \text{ or } \xstar=(\alpha, 2\alpha, 3\alpha, \ldots, n\alpha), \text{ with } f(\xstar) = \tilde{f}(\xstar) = -n\alpha\beta, \ \norm{\xstar-\xt[0]}^2\leq n^3/2.$$
Next, constrained to $x \in \Kl[n/2]$, i.e., $d\in \Kl[n/2]$, we have 
$$\min_{x \in \Kl[n/2]} \tilde{f}(x) = \min_{d\in \Kl[n/2]} \bar{f}(x) = -n\alpha\beta/2 \leq \min_{x \in \Kl[n/2]} f(x).$$
Thus the desired optimality lower bound follows immediately. 
\end{proof}

Now we ready to provide the lower communication complexity. 
\begin{theorem}
Let problem parameters $D_X^0,$ $\MPi[]$, $\Delta$ and a desired accuracy $\ep$ satisfying $\ep\leq \norm{\xstar- \xt[0]}\MPi[]/32$ be given. There is a communication network with a graph diameter $\Delta$, and a non-smooth hard instance $f$ with
$\norm{x_0 - \xstar} \leq \DX[0]$ and all $\myfi$ being $\MPi[]$-Lipschitz continuous such that the minimum number of communication rounds required of any black-box network optimization procedure to find an $\ep$-optimal solution is $(\DX\MPi/8\ep - 1)\Delta.$
\end{theorem}

\begin{proof}
This is a direct application of Lemma \ref{lm:lower_ns}. The hard instance $f$ is constructed according to Figure \ref{fig:ns_hard} with
\begin{itemize}[noitemsep]
\item $n$ being the smallest even integer larger than $\DX[0]\MPi[]/4\ep$ such that $n \leq \DX[0]\MPi[]/2\sqrt{2}\ep$,
\item $m=\Delta$, $\alpha=\sqrt{2}\DX[0]/n^{1.5}$ and $\beta=\MPi/2\sqrt{n}$.
\end{itemize}
Then it is easy to verify that the requirements for $f$ in the theorem statement are met. The desired lower bound of communication rounds can concluded by noticing that for any $t < (\DX\MPi/8\ep - 1)\Delta$ communication rounds, the output from any black-box procedure must satisfy
$$f(\xt) - f(\xstar)\geq n \alpha \beta /2 = \sqrt{2}\DX[0]\MPi[]/4n > \ep.$$
\end{proof}





==> lower_complexity.tex <==
\section{Lower Communication Complexity}
We construct the following smooth average cost problem to study the lower communication complexity:
\begin{equation}\label{eq:smb_obj}
\min_{x} \{f(x):= \underbrace{\gamma \sigma(x_0) + \tsum_{i=1}^{n/2} \sigma(x_{2i - 1} - x_{2i}) }_{\text{$f_l$ on the leftmost node}}+ \underbrace{\gamma \tsum_{i=0}^{n/2-1} \sigma(x_{2i} - x_{2i+1})+ \gamma x_n}_{\text{$f_r$ on the rightmost node}}\},\end{equation}
where $\sigma(\cdot)$ is a smoothed version of the absolute value function (Huber Loss function) parameterized by a positive constant $\tau$:
$$\sigma(y) := \begin{cases} \tfrac{1}{2\tau} \norm{y}^2 & \text{if } |y| \leq \tau, \\
|y| - \tau /2 & \text{otherwise}.
\end{cases}$$

Then the following properties of $f$ are easily verifiable:
\begin{lemma}\label{lm:lc_f_bsc_property}
Let $f$ be defined in \eqref{eq:smb_obj}, then an optimal solution $\xstar$ satisfies 
$$\xstar_0 = -\tau, \xstar_{j} = - (j +1)\tau\  \forall  j\geq 1,$$
with $f^* = - \tfrac{\gamma}{2}(n+1)\tau.$
\end{lemma}

\begin{proof}
The optimality can be easily verified with the first order condition $\grad_{x = \xstar} f(x) = 0.$
\end{proof}
Therefore if we define $X$ to be the ball with a radius $\norm{\xstar}$, upper bounds for the smoothness and Lipschitz constant of $f$ can also be easily verified. 
\begin{lemma}\label{lm:lc_eg_csts}
Let $X := \{{x \in \R^{n+1}: \norm{x} \leq \norm{\xstar}}\}$, then following upper bounds for the radius of $X$, Lipschitz constant and smoothness constant of $f$ over $2X$ hold:
$$\Rx \leq 2 \tau n \sqrt{n}, \Mf \leq 2\gamma\sqrt{n}, \Lf \leq 4 \gamma / \tau .$$
% \textcolor{red}{where $c$ is some universal constant. check the constant}
\end{lemma}
\begin{proof}
To derive the upper bound for $\Mf$, it suffices to note that every component of $\grad f(x)$ is bounded by $2 \gamma$ over $2X$. 
\end{proof}

Now we provide a lower bound for the optimality gap in $k$ communication rounds under the local information sharing framework proposed by \cite{scaman2017optimal}. With the loss of generality, assume that we start with $x^0 = 0$ at all nodes. Let $x_{(l)}, x_{(r)}$ \footnote{We use $x_{(i)}$ to differentiate solution at node $i$ from the $x_i$, the $i$th component of the solution variable $x$.} denote the local copy of solution $x$ at the leftmost and the rightmost node. Our analysis is based on the fact that starting from $[0,0]$, either a gradient update or a proximal update for $\gamma \sigma(x_{n} - x_{n-1})$ returns only $[0, 0]$. {}

First, the possible solutions to be generated proximal updates or gradient descent starting with $x^0$ must the following form, 
\begin{centering}
$x^0_l = [0, 0, \ldots, 0, 0]$ and $x^0_r = [0 , 0 ,\ldots , c_{n}]$ for some $c_n\in\R$.\end{centering}
Next, in order to generate a solution with $x_{n-1} \neq 0$, we must wait $\xbcr^0$ to be sent to the left node such that $\grad \gamma \sigma(x_{n} - x_{n-1})$ or proximal update of $\gamma \sigma(x_{n} - x_{n-1})$ can be evaluated with some non-zero $x_n$. So an $\xbcl$ with an non-zero $x_n$ can be found only in $\Delta$ communication rounds. Next, to generate a solution with a non-zero $x_{n-2}$, we need to send $\xbcl^{\Delta}$ back to the right node such that $\gamma \sigma(x_{n-1} - x_{n-2})$ can be evaluated with a non-zero $x_{n-1}$. Therefore, it takes $\Delta k$ communication rounds for a solution with nonzero $x_{n-k}, \ldots, x_{n}$ to be generated. This update pattern leads us to the following optimality gap. 

\begin{lemma}\label{lm:lower_opt_gap}
Starting from $x^0 = [0 , 0, \ldots, 0]$, if $X_{k\Delta}$ denote all the possible feasible solutions at all nodes in $k \Delta$ communication rounds with $k < n$, then 
$$\min_{x \in X_{k\Delta}}f(x) - f^* \geq \tfrac{\gamma}{2}(n -k)\tau.$$
\end{lemma}

\begin{proof}
As discussed above, every  $y \in X_{k\Delta}$ must have $y_0, y_1, \ldots, y_{n-k-1}$ being zero, thus 
$$f(y) = f_k(y) = \gamma \sigma(y_{n-k}) + \gamma \tsum_{i=n-k}^{n-1}\sigma(y_{i} - y_{i+1})+ \gamma y_n.$$
So the following $y^*$ satisfies the first order optimality condition 
$$y^*_{n-j} = \min\{(j -k -1)\tau + j ,0\}$$
with $f(y^*) = -\tfrac{k+1}{2}\tau \gamma$. The minimal optimality gap then follows from  subtracting the $f^*$ in Lemma \ref{lm:lc_f_bsc_property}.
\end{proof}

The following lower complexity bound for our example $f$ is then an easy consequence. 
\begin{proposition}
For any smoothness constant $\Lfbar$, radius $\Rxbar$ and normalized eigen-gap $\Delbar\geq 2$,  there exist a graph topology with a communication diameter less than $\Delbar$, a function $f$ with smoothness constant less than $\Lfbar$ and a feasible region less than $\Rxbar$ such that in $k\Delta$ communications rounds, the solution $y$ returned by any first order algorithm satisfy 

$$f(y) - f^* \geq c \tfrac{\Lfbar \Rxbar^2}{k^2},$$
where $c$ is some universal constant.
\end{proposition}

\begin{proof}
We can choose the linear graph with  $\floor{\Delbar} + 1$ nodes and a function of the form \eqref{eq:smb_obj} with 
$$n = 2k, \tau = \Rxbar / (n\sqrt{n}), \gamma = \Lfbar\tau /4.$$
Then by Lemma \ref{lm:lc_eg_csts}, the $f$ is a $\Lfbar$-smooth function and  its feasible region $X$ has a radius of $\Rxbar$. In addition Lemma \ref{lm:lower_opt_gap} implies that in $k\Delta$ communication rounds, a solution $y$ generated by any first order method satisfies 
$$\text{opt gap} \geq \tfrac{\gamma}{4}n\tau =  \tfrac{1}{16}(\tfrac{4\gamma}{\tau}) (n^3 \tau^2) \tfrac{1}{n^2} = \tfrac{1}{64}\tfrac{\Lfbar \Rxbar^2}{k^2}.$$
\end{proof}

Moreover, if we focus instead on constant $\Mpi$ and $\Rx$, we can recover a $\bigO\{1/n\}$ lower complexity. 
\begin{proposition}
For any Lipschitz constant $\Mfbar$, radius $\Rxbar$ and normalized eigen-gap $\Delbar\geq 2$,  there exist a graph topology with a communication diameter less than $\Delbar$, a smooth function $f$ with a Lipschitz constant $\Mfbar$ and a feasible region less than $\Rxbar$ such that in $k\Delta$ communications rounds, the solution $y$ returned by any first order algorithm satisfy 

$$f(y) - f^* \geq c \tfrac{\Mfbar \Rxbar}{k},$$
where $c$ is some universal constant.
\end{proposition}

\begin{proof}
We can choose the linear graph with  $\floor{\Delbar} + 1$ nodes and a function of the form \eqref{eq:smb_obj} with 
$$n = 2k, \tau = \Rxbar / (n\sqrt{n}), \gamma = \Mfbar /2\sqrt{n}.$$
Then by Lemma \ref{lm:lc_eg_csts}, then smooth function $f$ is a $\Mfbar$-smooth function and  its feasible region $X$ has a radius of $\Rxbar$. In addition Lemma \ref{lm:lower_opt_gap} implies that in $k\Delta$ communication rounds, a solution $y$ generated by any first order method satisfies 
$$\text{opt gap} \geq \tfrac{\gamma}{4}n\tau =  \tfrac{1}{16 n}(2\gamma\sqrt{n})(2 \tau n \sqrt{n}) \geq \tfrac{1}{32} \tfrac{\Mfbar \Rxbar}{n}.$$
\end{proof}

%maybe the role of max is to emphasize that the constant dependency is with respect to the local maximal rather than global






==> robust.tex <==
\section{A Communication Efficient Distributed Algorithm for Robust Optimization}

We propose in this section a communication efficient algorithm for solving robust optimization in a distributed network. More specifically, consider 
\begin{equation}\label{eq:robust_prob}
\min_{x \in X}\{f(x) := \max\{\SubAddi{g}{1}(x), \SubAddi{g}{2}(x), \ldots, \SubAddi{g}{m}(x) \} \equiv \max_{p \in \Delta_+^m} \sumi \mypi\gi(x) \},
\end{equation}
where the cost function $\SubAddi{g}{i}$ is local to node $i$ in the communication network. We impose the following assumptions regarding its structure.
\begin{assumption}
\begin{enumerate}
\item Each local cost function $\SubAddi{g}{i}$ is defined on $\R^n$. They are all convex and $\Mpi$-Lipschitz continuous.
\item The proximal update associated with each $\SubAddi{g}{i}$ can be efficiently computed, i.e., 
$$\SubAddi{\bxht}{i} \leftarrow \argmin_{x\in R^n} \gi(x) + \tfrac{\tau}{2} \normsq{x - \xbar}
  \forall \tau \geq 0, \xbar \in \R^n, i \in [m].$$
\item $X$ is a convex and compact set with $\Dx := \max_{x_1, x_2 \in X} \norm{x_1 - x_2} < \infty. $
\end{enumerate}
\end{assumption}
\textcolor{red}{We will try to relax the assumptions in later sections, for e.g. the proximal update of g.}

Our algorithmic development is inspired by \cite{zhang2019efficient}. In \cite{zhang2019efficient}, the authors use Fenchel conjugate of $\gi$ to reformulated \ref{eq:robust_prob} as a ``min-max-max'' saddle point problem
\begin{equation}
\min_{x \in X} \max_{p \in \Delta_+^m} \max_{\pii \in \Pii} \{\La(x; p, \pi):= \max_{p \in \Delta_+^m} \sumi p_i\inner{\pii}{x} - \gi^*(\pii) \},
\end{equation}
where $\gi^*(\pii):= \max_{x \in \R^n} \inner{\pii}{x} - \gi(x)$ and $\Pii := \dom(\gi^*).$ They propose to solve the saddle point problem approximately by the following proximal updates in each iteration:
 \begin{enumerate}[leftmargin=2cm]
 \small
    \item[[$\pi$ update]] Set $\piit := \argmax_{\pii \in \Pii} \inner{\pii}{\xtt + \thetat(\xtt - \xttt) } - \gi^*(\pii) + \tfrac{\taut}{2} \normsq{\pii - \addtt\pii}.$
    \item[[$p$ update]] Set $\pt := \argmax_{\myp \in \Delta^+} \sumi \mypi \left(\inner{\piit}{\xtt} + \thetat\inner{\piitt}{\xtt - \xttt} - \gi^*(\piit)\right) + \gamt D(\myp||\addtt\myp).$
    \item[[$x$ update]] Set $\xt = \argmin_{x \in X} \inner{x}{\sumi \addt\mypi \piit} + \tfrac{\etat}{2}\normsq{x - \xtt}.$
  \end{enumerate} 
Our task consists in implementing those proximal updates in a distributed network and  keeping control of the error resulted from using local decision variables. More specifically, we let each local node to keep their own $\{\bxit; \addt\pitl, \piit\}_{t}$, where $\addt\pitl$ represent some unnormalized probability mass.
Clearly if we use the ComAvg Algorithm to ensure consistency among all $\{\bxt\}$, the $\pi$ update can be implemented in a distributed network easily (Line 2 in Algorithm \ref{alg:ACSD}). As for the $p$ update, we utilize the fact that the proximal update with entropy Bregman distance $D(\cdot||\addtt{p})$  is the same as softmax. If $g^t:=\inner{\piit}{\xtt} + \thetat\inner{\piitt}{\xtt - \xttt} - \gi^*(\piit)$, then the $p$ update is equivalent to 
$$\Addit\myp := \Additt\myp \exp(g^t_{\bci}) / \sumi \Additt\myp \exp(g^t_{\bci}).$$
Thus the unnormalized $\addt\pitl$ can be computed locally in Line 3 of Algorithm \ref{alg:ACSD}. 
Next, the $x$ update requires the normalized probability mass $\addt\mypi $ when calculating $\sumi \addt\mypi \piit$. So Line 4 of Algorithm \ref{alg:ACSD} utilizes ComAvg Algorithm to find the normalizing constant $$\addt\bsi \approx \sumi \pitl /m$$
 and then perform the $x$ proximal update like Algorithm \ref{alg:ACAGD}.


% \begin{minipage}{1\textwidth}
\begin{algorithm}[htb!]
\caption{Almost Consistent SD}
\label{alg:ACSD}
\begin{algorithmic}[1]
\Require $\AddiO{\bxbr} = \AddiO{\bx} = \addO{x} \in X, \forall i \in [m] $. Non-negative step-sizes $\{\sadt\theta, \sadt\tau, \sadt\gamma, \sadt\eta\}_{t=1}^N$.

\For{$t =  1,2,3, ... N$}
\parState{For each node $i$, set $\Addit\bxtl = \Additt\bx + \sadt\thetat (\Additt\bx - \Addi{\addttt\bx})$. \\
Compute $\addt\byi = \argmin_{y \in \R^n} \gi(y) + \tfrac{1}{\sadt\tau} \normsq{\addt\bxtl + \sadt\gamma \addtt\pii - y}$ and set $\addt\pii:= \addtt\pii - \tfrac{1}{\sadt\tau}(\addt\byi- \Addit\bxtl)$.\\
Compute $\bgi^*(\piit):= \inner{\piit}{\Addit\bxtl + \taut \addtt\pii} - \gi(\Addit\by).$  }
\parState{For every node $i$, compute $\addt{\tilde{g}} = \inner{\piit}{\bxitt} - \thetat \inner{\addtt\pii}{\bxitt - \bxittt} - \bgi^*(\piit).$\\
Set $\addt\pitl = \addtt\pitl \exp(\addt{\tilde{g}}/\gamt).$ }
\parState{Compute $\{\addt\bsi\}$ by running ComAvg initialized to $[\pitl[1], \pitl[2], \ldots, \pitl[m]]$ till $\devi{\tfrac{1}{\addt\bsav} \addt\mybs} \leq \ep_s \leq 1/4$.\\
Set $\Addit\bxud = \Additt\bx - \tfrac{1}{\etat} (\addt\pitl \piit/ \addt\bsi).$ Compute $\{\Addit\bxht\}$ by running ComAvg initialized to $[\addt\bxud_{\bci[1]}, \addt\bxud_{\bci[2]}, \ldots, \addt\bxud_{\bci[m]}]$  until $\devi{\addt\bxht} \leq \ep_x \leq 1$. Set $\bxit = \projX{\Addit\bxht}$.}
\EndFor\\
\Return $\AddiN\bxbr = \sumt \bxit / N.$
\end{algorithmic}
\end{algorithm}
% \end{minipage}
\subsection{Approximate Three Point Inequalities}
We show in this subsection that the iterates generated satisfies the three point inequalities for $x$, $p$ and $\pi$ proximal updates approximately. 

\begin{proposition}
The $\{\addt\pi\}$ generated by Algorithm \ref{alg:ACSD} satisfies the following the approximate three point inequality, 
\begin{equation}
\begin{split}
\inner{\Addavt\bxtl}{\pii - \Addit\pi}& - \gi^*(\pii) + \gi^*(\Addit{\pi})\ + \tfrac{\taut}{2} \normsq{\piitt - \piit} + \tfrac{\taut}{2} \normsq{\piitt - \piit} \\
 &\leq \tfrac{\taut}{2} \normsq{\piitt - \piit} + \delpit \quad \quad  \forall \pii \in \Pii, \forall i \in [m],
 \end{split}
\end{equation}
with $|\delpit|  \leq 2 \Mpi \devi{\addt\bxtl} \leq (2 + 4\thetat)\Mpi \ep_x$.
\end{proposition}

\begin{proof}

\end{proof}

\begin{proposition}
If $\hat{g}^t$ denotes the predicted cost for the average solution generated by Algorithm \ref{alg:ACSD},
{\centering $\ghtt:= [\ghtt_{\bci[1]}, \ghtt_{\bci[2]}, \ldots, \ghtt_{\bci[m]}]$ where $\ghtt_{\bci}:= \inner{\piit}{ \Addavtt\bx} + \thetat \inner{\piitt}{ \Addavtt\bx - \Addavttt\bx} - \gi^*(\piit), $}
then the normalized probability mass $\pt := \tfrac{1}{\sumi \addt\pitl} \addt\ptl$  satisfies 
\begin{equation}
\sumi \ghtt_{\bci} (\mypi - \addt\mypi) + \taut (D(\myp|| \pt) + D(\pt|| \ptt) - D(\myp|| \ptt)) \leq \delpt \quad \forall \myp \in \Delta^+,
\end{equation}
where $|\delpt| \leq (1 + 2\thetat) \Mpi \ep_x $
\end{proposition}

\begin{proposition}
Let $\{\bxt\}$ be generated by Algorithm \ref{alg:Avg1} and let $\pt := \tfrac{1}{\sumi \addt\pitl} \addt\ptl$. Then the averaged solution $\{\Addavt\bx\}$ satisfies 
\begin{equation}
\inner{\Addavt\bx - x}{\sumi \Addit\myp \piit} +\tfrac{\etat}{2} (\normsq{\Addavt \bx - x} + \normsq{\Addavtt \bx - \Addavt \bx} - \normsq{\Addavtt\bx - x}) \leq \delxt,
\end{equation}
where $|\delxt| \leq 2 \Dx \Mpi \ep_s + \frac{\etat}{m} \ep_x^2.$
\end{proposition}
\subsection{Convergence Analysis}
We put the preceding approximate three point inequalities together to analyze Algorithm \ref{alg:ACSD}`s convergence. The analysis is similar to those in \cite{zhang2019efficient} in that we first prove the convergence in some gap function and then use gap function to bound the optimality gap in $f$. 

More specifically, consider the following gap function for $\zt = (\Addavt\bx; \pt, \addt\pi)$,
$$Q(\zt, z):= \La(\xt;\myp, \pi) - \La(x; \pt, \pi^t)$$
  where $z=(x;\myp, \pi)$ is some feasible reference point in $X\times \Delta_+ \times \prod_{i=1}^{m} \Pii$. Notice that $Q(\bar{z}, z) \leq 0\ \forall z$ if $\bar(z)$ is a saddle point. We establish the suboptimality of $\AddavN\bx$ returned by Algorithm \ref{alg:ACSD} by showing the convergence of the partial sum $\sumt Q(\zt; z)$ for all $z$ in the next proposition.
\begin{proposition}
Let $\{\Addavt\bx, \addt\myp, \addt\pi\}$ be generated by Algorithm \ref{alg:ACSD} with constant stepsize satisfying 
\end{proposition}

Towards that end, we decompose $Q$ into three components related to the optimality of $x,p,\pi$ respectively, i.e., $Q(\zbar;z) \equiv Q_x(\zbar;z) + Q_p(\zbar;z) + Q_\pi(\zbar;z)$ where
\begin{equation}\label{eq:three_part}
\begin{split}
&Q_\pi(\zbar;z) := \La(\bar{x}; \myp, \pi) - \La(\bar{x}; \myp, \bar{\pi}) = \sumi \mypi \inner{\bar{x}}{\pii - \bar{\pi}_{\bci}} - \gi^*(\pii) + \gi^*(\bar{\pi}_{\bci}).\\
&Q_p(\zbar;z) := \La(\bar{x}; \myp, \bar{\pi}) - \La(\bar{x}; \bar{\myp}, \bar{\pi}) = \sumi (\mypi - \bar{\myp}_{\bci}) \inner{\bar{x}}{\bar{\pi}_{\bci}} -  \gi^*(\bar{\pi}_{\bci}).\\
&Q_x(\zbar;z) := \La(\bar{x}; \bar{\myp}, \bar{\pi}) - \La(x; \bar{\myp}, \bar{\pi}) = \inner{\sumi \bar{\myp}_{\bci}\bar{\pi}_{\bci}}{\bar{x} - x} .\\ 
\end{split}
\end{equation}
































